Integrable Whole-body Orientation Coordinates for Legged Robots

Complex multibody legged robots can have complex rotational control challenges. In this paper, we propose a concise way to understand and formulate a \emph{whole-body orientation} that (i) depends on system configuration only and not a history of motion, (ii) can be representative of the orientation of the entire system while not being attached to any specific link, and (iii) has a rate of change that approximates total system angular momentum. We relate this orientation coordinate to past work, and discuss and demonstrate, including on hardware, several different uses for it.

==> background.tex <==

I think starting with simple examples before showing 3D rotation frame is kinda awkward, so I'll show Nadia and the 3D frames first. I want to tell people the high level objective first.

\subsection{2D and 3D translation}


\subsection{2D rotation}

2D rotation is a 1D problem.

Simple stick figure. 3 link robot. One torso and two legs.

The weighted sum of each link's angles for 2D rotation is a good choice but it could be better. It depend on your task.
Even 2D rotatoin, the path integral is still path dependent. (like my 3-link exame, and Gabe's simple example) 
 



